Relativistic (or $2$-prover $1$-round) zero-knowledge protocol for $\mathsf{NP}$ secure against quantum adversaries

In this paper, we show that the zero-knowledge construction for Hamiltonian cycle remains secure against quantum adversaries in the relativistic setting. Our main technical contribution is a tool for studying the action of consecutive measurements on a quantum state which in turn gives upper bounds on the value of some entangled games. This allows us to prove the security of our protocol against quantum adversaries. We also prove security bounds for the (single-round) relativistic string commitment and bit commitment in parallel against quantum adversaries. As an additional consequence of our result, we answer an open question from [Unr12] and show tight bounds on the quantum knowledge error of some $\Sigma$-protocols.

==> new_macros.tex <==
\newtheorem{theorem}{Theorem}
\newtheorem{conjecture}{Conjecture}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{claim}{Claim}
\newtheorem{openprob}{Open Problem}
\newtheorem{remk}{Remark}
\newtheorem{apdxlemma}{Lemma}

\newenvironment{remark}{\begin{remk}

\begin{normalfont}}{\end{normalfont}
\end{remk}}
\newtheorem{sublemma}[theorem]{Sublemma}


%%%%%%%%%%%%%%%%%%%% proof environments

\def\FullBox{\hbox{\vrule width 8pt height 8pt depth 0pt}}

\def\qed{\ifmmode\qquad\FullBox\else{\unskip\nobreak\hfil
\penalty50\hskip1em\null\nobreak\hfil\FullBox
\parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}


\newenvironment{proof}{\begin{trivlist} \item {\bf Proof:~~}}
  {\qed\end{trivlist}}


\newtheorem{fact}[theorem]{Fact}

\def\qedsketch{\ifmmode\Box\else{\unskip\nobreak\hfil
\penalty50\hskip1em\null\nobreak\hfil$\Box$
\parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}

\newenvironment{proofsketch}{\begin{trivlist} \item {\bf
Proof Sketch:~~}}
  {\qedsketch\end{trivlist}}

\newenvironment{proofof}[1]{\begin{trivlist} \item {\bf Proof
#1:~~}}
  {\qed\end{trivlist}}

\newenvironment{claimproof}{\begin{quotation} \noindent
{\bf Proof of claim:~~}}{\qedsketch\end{quotation}}


%%%%%%%%%%%%%%%%%%%%%%% text macros
\newcommand{\etal}{{\it et~al.\ }}
\newcommand{\ie} {{\it i.e.\ }}
\newcommand{\eg} {{\it e.g.\ }}
\newcommand{\cf}{{\it cf.\ }}

%%%%%%%%%%%%%%%%%%%%%%% general useful macros
\newcommand{\eqdef}{\mathbin{\stackrel{\rm def}{=}}}
\newcommand{\R}{{\mathbb R}}
\newcommand{\N}{{\mathbb{N}}}
% \newcommand{\Z}{{\mathbb Z}}
\newcommand{\poly}{{\mathrm{poly}}}
\newcommand{\loglog}{{\mathop{\mathrm{loglog}}}}
\newcommand{\zo}{\{0,1\}}
\newcommand{\suchthat}{{\;\; : \;\;}}
\newcommand{\pr}[1]{\Pr\left[#1\right]}
\newcommand{\deffont}{\em}
\newcommand{\getsr}{\mathbin{\stackrel{\mbox{\tiny R}}{\gets}}}
\newcommand{\E}{\mathop{\mathbb E}\displaylimits}
\newcommand{\Var}{\mathop{\mathrm Var}\displaylimits}
\newcommand{\eps}{\varepsilon}
\newcommand{\KL}{\mathop{\mathrm {KL}}\displaylimits}
\newcommand{\Ent}{\mathrm H}
\newcommand{\KLb}{\mathop{\mathrm{KL_2}}}
\newcommand{\Supp}{\mathop{\mathrm{Supp}}\displaylimits}
\newcommand{\XOR}{\textsc{XOR}}
\newcommand{\OR}{\textsc{OR}}
\newcommand{\AND}{\textsc{AND}}
\newcommand{\wt}{\mathrm{wt}}
\newcommand{\Disj}{\mathop{\mathrm{Disj}}\displaylimits}
\newcommand{\mDisj}{\mathop{\mathrm{MutDisj}}\displaylimits}

%%%%%%%%%%%%%%%%%%% macros particular to this course
% for author notes
\ifnum\draft=1
\newcommand{\authnote}[2]{{ \bf [#1's Note: #2]}}
\else
\newcommand{\authnote}[2]{}
\fi
\newcommand{\Snote}[1]{{\authnote{Salil}{#1}}}
\newcommand{\Fnote}[1]{{\authnote{Florin}{#1}}}

\newcommand{\SZKOWFchar}{\textrm{SZK/OWF Characterization}}
\newcommand{\NISZKhOWFchar}{\textrm{NISZK$^h$/OWF Characterization}}
\newcommand{\NIZKbold}{\textbf{NIZK}}
\newcommand{\NISZKbold}{\textbf{NISZK}}
\newcommand{\ZKbold}{\textbf{ZK}}
\newcommand{\SZKbold}{\textbf{SZK}}

\def\textprob#1{\textmd{\textsc{#1}}}
\newcommand{\mathprob}[1]{\mbox{\textmd{\textsc{#1}}}}
\newcommand{\SAT}{\mathprob{SAT}}
\newcommand{\yes}{{\sc yes}}
\newcommand{\no}{{\sc no}}
\newcommand{\QuadRes}{\textprob{Quadratic Residuosity}}
\newcommand{\GraphIso}{\textprob{Graph Isomorphism}}
\newcommand{\GraphNoniso}{\textprob{Graph Nonisomorphism}}
\newcommand{\SZKOWFcond}{\textprob{SZK/OWF Condition}}
\newcommand{\NISZKhOWFcond}{\textprob{NISZK$^h$/OWF Condition}}
\newcommand{\NISZKcrsOWFcond}{\textprob{NISZK$^{crs}$/OWF Condition}}
\newcommand{\NISZKpubOWFcond}{\textprob{NISZK$^{pub}$/OWF Condition}}
\newcommand{\CIIDC}{\mathprob{CIIDC}}
\newcommand{\IID}{\mathprob{IID}}
\newcommand{\StatDiffUni}{\textprob{Statistical Difference from Uniform}}
\newcommand{\StatDiff}{\textprob{Statistical Difference}}
\newcommand{\CondEntApp}{\textprob{Conditional Entropy Approximation}}
\newcommand{\EntDiff}{\textprob{Entropy Difference}}
\newcommand{\EntApp}{\textprob{Entropy Approximation}}
\newcommand{\IndCond}{\textprob{Indistinguishability Condition}}
\newcommand{\CondPsEnt}{\textprob{Conditional Pseudoentropy Condition}}
\newcommand{\CondIIDCond}{\textprob{Computational Image Intersection Density Condition}}
\newcommand{\ImageInt}{\textprob{Image Intersection Density}}


\newcommand{\class}[1]{\mathrm{#1}}
\newcommand{\BPP}{\class{BPP}}
\newcommand{\NP}{\class{NP}}
\renewcommand{\P}{\class{P}}
\newcommand{\negl}{{\mathrm{neg}}}
\newcommand{\SZK}{\class{SZK}}
\newcommand{\CZK}{\class{ZK}}
\newcommand{\ZK}{\CZK}
\newcommand{\SZKh}{\class{SZK}^\mathrm{h}}
\newcommand{\CZKh}{\class{ZK}^\mathrm{h}}
\newcommand{\ZKh}{\CZKh}
\newcommand{\SZKpub}{\class{SZK}^\mathrm{pub}}
\newcommand{\CZKpub}{\class{ZK}^\mathrm{pub}}
\newcommand{\SZKcrs}{\class{SZK}^\mathrm{crs}}
\newcommand{\CZKcrs}{\class{ZK}^\mathrm{crs}}
\newcommand{\NISZKh}{\class{NISZK}^\mathrm{h}}
\newcommand{\NISZKcrs}{\class{NISZK}^\mathrm{crs}}
\newcommand{\NISZKpub}{\class{NISZK}^\mathrm{pub}}
\newcommand{\NISZK}{\class{NISZK}}
\newcommand{\NICZKh}{\class{NIZK}^\mathrm{h}}
\newcommand{\NICZKcrs}{\class{NIZK}^\mathrm{crs}}
\newcommand{\NICZKpub}{\class{NIZK}^\mathrm{pub}}
\newcommand{\NICZK}{\class{NIZK}}
\newcommand{\NIZK}{\NICZK}
\newcommand{\NIZKh}{\NICZKh}
\newcommand{\NIZKpub}{\NICZKpub}
\newcommand{\NIZKcrs}{\NICZKcrs}
\newcommand{\IP}{\class{IP}}
\newcommand{\AM}{\class{AM}}
\newcommand{\PSPACE}{\class{PSPACE}}
\newcommand{\Com}{\class{Com}}
\newcommand{\view}{\class{view}}

\newcommand{\Enc}{E}
\newcommand{\Dec}{D}
\newcommand{\Gen}{G}
\newcommand{\Tag}{M}
\newcommand{\Sign}{\mathrm{Sign}}
\newcommand{\Ver}{V}
\newcommand{\Commit}{\mathrm{Com}}

\newcommand{\MsgSp}{\mathcal{P}}
\newcommand{\KeySp}{\mathcal{K}}
\newcommand{\CiphSp}{\mathcal{C}}

\newcommand{\key}{k}
\newcommand{\td}{t}

\newcommand{\DIV}{\mathrm{DIV}}
\newcommand{\EXP}{\mathrm{EXP}}
\newcommand{\MODEXP}{\mathrm{MODEXP}}
\newcommand{\GCD}{\mathrm{GCD}}


\newcommand{\Dist}{\mathcal{D}}
\newcommand{\LR}{\mathrm{LR}}
\newcommand{\Oracle}{\mathrm{Oracle}}
\newcommand{\Adv}{\mathrm{Adv}}
\newcommand{\DES}{\mathrm{DES}}
\newcommand{\AES}{\mathrm{AES}}
\newcommand{\FFam}{\mathcal{F}}
\newcommand{\HFam}{\mathcal{H}}
\newcommand{\Rand}{\mathcal{R}}
\newcommand{\Ind}{\mathcal{I}}
\newcommand{\Dom}{D}
\newcommand{\Rng}{R}
\newcommand{\DLog}{\mathrm{DLog}}
\newcommand{\QR}{\mathrm{QR}}
\newcommand{\half}{\mathrm{half}}
\newcommand{\lsb}{\mathrm{lsb}}
\newcommand{\IV}{\mathrm{IV}}
\newcommand{\Field}{\mathbb{F}}
\newcommand{\PK}{\mathit{PK}}
\newcommand{\SK}{\mathit{SK}}
\newcommand{\pk}{\mathit{pk}}
\newcommand{\sk}{\mathit{sk}}
% \newcommand{\key}{\mathsf{key}}

\newcommand{\accept}{\mathtt{accept}}
\newcommand{\reject}{\mathtt{reject}}
\newcommand{\fail}{\mathtt{fail}}
\newcommand{\MD}[1]{\mathrm{MD{#1}}}
\newcommand{\SHA}{\mbox{SHA-1}}

\newcommand{\pf}{\mathit{proof}}
\newcommand{\compind}{\mathbin{\stackrel{\rm
c}{\equiv}}}

\newcommand{\Ideal}{\mathbf{Ideal}}
\newcommand{\Real}{\mathbf{Real}}
\newcommand{\mvec}{\overline{m}}

% Added by A.Chailloux : Quantum classes and other
\newcommand{\BQP}{\class{BQP}}
\newcommand{\QSZK}{\class{QSZK}}
\newcommand{\HVQSZK}{\class{HVQSZK}}
\newcommand{\QNISZK}{\class{QNISZK}}
\newcommand{\QNIPZK}{\class{QNIPZK}}
\newcommand{\QEA}{\textsc{QEA}}
\newcommand{\QED}{\textsc{QED}}
\newcommand{\QSD}{\textsc{QSD}}
\newcommand{\QSCU}{\textsc{QSCU}}
%\newcommand{\SCU}{\textsc{SCU}}
\newcommand{\SCUq}{\textsc{SCU}^\mathrm{q}}
\newcommand{\SD}{\mathrm{\Delta}}
\newcommand{\SC}{\mathrm{\Gamma}}
\newcommand{\SDp}{\textsc{SD}} % The promise problem SD
\newcommand{\mIID}{\mathprob{IID}}
\newcommand{\ED}{\textsc{ED}}
\newcommand{\EA}{\textsc{EA}}
\newcommand{\EAbar}{\overline{\mathprob{EA}}}
\newcommand{\SCU}{\textsc{SCU}}

\newcommand{\QNISZKh}{\class{QNISZK}^\mathrm{h}}
\newcommand{\QSZKh}{\class{QSZK}^\mathrm{h}}
\newcommand{\QAZK}{\textrm{weak-}\class{QSZK}}
\newcommand{\QNISZKch}{\class{QNISZK}^\mathrm{ch}}
\newcommand{\QNISZKhNU}{\class{QNISZK}^\mathrm{mh}}
\newcommand{\NISZKsec}{\class{NISZK}^\mathrm{sec}}
\newcommand{\IIDq}{\class{IID}^\mathrm{q}}
\newcommand{\HVSZK}{\class{HVSZK}}
\newcommand{\HVSZKq}{\class{HVSZK}^\mathrm{q}}
\newcommand{\SZKq}{\class{SZK}^\mathrm{q}}
\newcommand{\QNISZKcrs}{\class{QNISZK}^\mathrm{crs}}

\newcommand{\COMMENT}[1]{}
\newcommand{\ket}[1]{|#1\rangle}
\newcommand{\bra}[1]{\langle#1|}
\newcommand{\ketbra}[2]{|#1\rangle\langle#2|}
\newcommand{\inp}[2]{\langle{#1}|{#2}\rangle} % inproduct, < | >
\def\01{\{0,1\}}
\newcommand{\braket}[2]{\langle{#1}|{#2}\rangle} % inproduct, < | >
\def\01{\{0,1\}}
\newcommand{\prot}[1]{\langle {#1} \rangle}
\newcommand{\triple}[3]{\langle{#1}|{#2}|{#3}\rangle}

\newcommand{\zk}{Zero-Knowledge }
\newcommand{\un}{\mathcal{U}}

\newcommand{\norm}[1]{\mbox{$\parallel{#1}\parallel$}}
\newcommand{\Tr}{\mbox{\rm Tr}}

\newcommand{\maj}[2]{\mathrm{Maj_{#1}(#2)}}
\newcommand{\wdt}[1]{\widetilde{#1}}

\newcommand{\cadre}[1]
{
\begin{tabular}{|p{15.4cm}|}
\hline
#1 \\
\hline
\end{tabular}
}

%New paper

\newcommand{\spB}{\mathcal{B}}
\newcommand{\spR}{\mathcal{R}}
\newcommand{\spH}{\mathcal{H}}
\newcommand{\spa}[1]{\mathcal{#1}}

\newcommand{\spall}{\spa{P} \otimes \spa{B} \otimes \spa{V} \otimes \spa{W}}

\newcommand{\str}{tr}

\newcommand{\css}{CS-Security }
\newcommand{\sits}{{SIT-Security }}

\newcommand{\QSZKcs}{\class{QSZK}_\mathrm{cs}}

\newcommand{\enc}{\eps}

\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\Z}{\mathcal{Z}}
\newcommand{\I}{\mathcal{I}}

\newcommand{\Id}{\mathbb{I}}

\newcommand{\red}{\preccurlyeq}

\newcommand{\lin}[1]{\mathcal{L}(#1)}

\newcommand{\cond}{S_c}

\newcommand{\pp}{{\textbf{P1}}}
\newcommand{\qq}{{\textbf{P2}}}

\newcommand{\Abort}{{\mathrm{Abort}}}

